Reconstructing the shock history in the CMZ of NGC 253 with ALCHEMI

HNCO and SiO are well known shock tracers and have been observed in nearby galaxies, including the nearby (D=3.5 Mpc) starburst galaxy NGC 253. The simultaneous detection of these two species in regions where the star formation rate is high may be used to study the shock history of the gas. We perform a multi-line molecular study using these two shock tracers (SiO and HNCO) with the aim of characterizing the gas properties. We also explore the possibility of reconstructing the shock history in NGC 253's Central Molecular Zone (CMZ). Six SiO transitions and eleven HNCO transitions were imaged at high resolution $1''.6$ (28 pc) with the Atacama Large Millimeter/submillimeter Array (ALMA) as part of the ALCHEMI Large Programme. Both non-LTE radiative transfer analysis and chemical modelling were performed in order to characterize the gas properties, and to investigate the chemical origin of the emission. The non-LTE radiative transfer analysis coupled with Bayesian inference shows clear evidence that the gas traced by SiO has different densities and temperatures than that traced by HNCO, with an indication that shocks are needed to produce both species. Chemical modelling further confirms such a scenario and suggests that fast and slow shocks are responsible for SiO and HNCO production, respectively, in most GMCs. We are also able to infer the physical characteristics of the shocks traced by SiO and HNCO for each GMC. Radiative transfer and chemical analysis of the SiO and HNCO in the CMZ of NGC 253 reveal a complex picture whereby most of the GMCs are subjected to shocks. We speculate on the possible shock scenarios responsible for the observed emission and provide potential history and timescales for each shock scenario. Higher spatial resolution observations of these two species are required in order to quantitatively differentiate between scenarios.

==> ALCHEMI_AuthorList.tex <==
%% A significant change from earlier AASTEX versions is in the structure for 
%% calling author and affiliations. The change was necessary to implement 
%% auto-indexing of affiliations which prior was a manual process that could 
%% easily be tedious in large author manuscripts.
%%
%% The \author command is the same as before except it now takes an optional
%% argument which is the 16 digit ORCID. The syntax is:
%% \author[xxxx-xxxx-xxxx-xxxx]{Author Name}
%%
%% This will hyperlink the author name to the author's ORCID page. Note that
%% during compilation, LaTeX will do some limited checking of the format of
%% the ID to make sure it is valid. If the "orcid-ID.png" image file is 
%% present or in the LaTeX pathway, the OrcID icon will appear next to
%% the authors name.
%%
%% Use \affiliation for affiliation information. The old \affil is now aliased
%% to \affiliation. AASTeX v6.3 will automatically index these in the header.
%% When a duplicate is found its index will be the same as its previous entry.
%%
%% Note that \altaffilmark and \altaffiltext have been removed and thus 
%% can not be used to document secondary affiliations. If they are used latex
%% will issue a specific error message and quit. Please use multiple 
%% \affiliation calls for to document more than one affiliation.
%%
%% The new \altaffiliation can be used to indicate some secondary information
%% such as fellowships. This command produces a non-numeric footnote that is
%% set away from the numeric \affiliation footnotes.  NOTE that if an
%% \altaffiliation command is used it must come BEFORE the \affiliation call,
%% right after the \author command, in order to place the footnotes in
%% the proper location.
%%
%% Use \email to set provide email addresses. Each \email will appear on its
%% own line so you can put multiple email address in one \email call. A new
%% \correspondingauthor command is available in V6.3 to identify the
%% corresponding author of the manuscript. It is the author's responsibility
%% to make sure this name is also in the author list.
%%
%% While authors can be grouped inside the same \author and \affiliation
%% commands it is better to have a single author for each. This allows for
%% one to exploit all the new benefits and should make book-keeping easier.
%%
%% If done correctly the peer review system will be able to
%% automatically put the author and affiliation information from the manuscript
%% and save the corresponding author the trouble of entering it by hand.

% INSERT MAIN AUTHORS FOR ARTICLE HERE BEFORE CORE ALCHEMI

% You will also need to adjust the number of authors listed on the first page by adding number of main authors to collaboration command below

% Also do not forget to reorder email listing in emaillist.tex file to reflect order here
\author[0000-0002-1227-8435]{Ko-Yun Huang}
\affiliation{Leiden Observatory, Leiden University, PO Box 9513, NL-2300 RA Leiden, The Netherlands}
%
\author[0000-0003-4025-1552]{Jonathan Holdship}
\affiliation{Leiden Observatory, Leiden University, PO Box 9513, NL-2300 RA Leiden, The Netherlands}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT}
%
\author[0000-0001-8504-8844]{Serena Viti}
\affiliation{Leiden Observatory, Leiden University, PO Box 9513, NL-2300 RA Leiden, The Netherlands}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT}
%
\author[0000-0003-1183-9293]{Jeffrey G.~Mangum}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Road,
  Charlottesville, VA  22903-2475, USA}
%\email{jmangum@nrao.edu}
%
\author[0000-0002-2333-5474]{Erica Behrens}
\affiliation{Department of Astronomy, University of Virginia, P.~O.~Box 400325, 530 McCormick Road, Charlottesville, VA 22904-4325}

\author[0000-0002-6824-6627]{Nanase Harada}
\affiliation{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\affiliation{Department of Astronomy, School of Science, The Graduate University for Advanced Studies (SOKENDAI), 2-21-1 Osawa, Mitaka, Tokyo, 181-1855 Japan}


\author[0000-0001-9281-2919]{Sergio Mart\'in}
\affiliation{European Southern Observatory, Alonso de C\'ordova, 3107, Vitacura, Santiago 763-0355, Chile}
\affiliation{Joint ALMA Observatory, Alonso de C\'ordova, 3107, Vitacura, Santiago 763-0355, Chile}
%\email{Sergio.Martin@eso.org}

\author[0000-0001-5187-2288]{Kazushi Sakamoto}
\affiliation{Institute of Astronomy and Astrophysics, Academia Sinica, 11F of AS/NTU
Astronomy-Mathematics Building, No.1, Sec. 4, Roosevelt Rd, Taipei 10617, Taiwan}
%\email{ksakamoto@asiaa.sinica.edu.tw}

\author[0000-0002-9931-1313]{Sebastien Muller}
\affiliation{Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, SE-43992 Onsala, Sweden}
%\email{mullers@chalmers.se}

\author[0000-0001-8153-1986]{Kunihiko Tanaka}
\affil{Department of Physics, Faculty of Science and Technology, Keio University, 3-14-1 Hiyoshi, Yokohama, Kanagawa 223--8522 Japan}
%\email{ktanaka@phys.keio.ac.jp}

\author[0000-0002-6939-0372]{Kouichiro Nakanishi}
\affiliation{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\affiliation{Department of Astronomy, School of Science, The Graduate University for Advanced Studies (SOKENDAI), 2-21-1 Osawa, Mitaka, Tokyo, 181-1855 Japan}
%\email{nakanisi.k@nao.ac.jp}

\author[0000-0002-7758-8717]{Rub\'en~Herrero-Illana}
\affiliation{European Southern Observatory, Alonso de C\'ordova, 3107, Vitacura, Santiago 763-0355, Chile}
\affiliation{Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Magrans, E-08193 Barcelona, Spain}
%\email{rherrero@eso.org}

\author{Yuki Yoshimura}
\affiliation{Institute of Astronomy, Graduate School of Science,
The University of Tokyo, 2-21-1 Osawa, Mitaka, Tokyo 181-0015, Japan}
%\email{yyoshimura@ioa.s.u-tokyo.ac.jp}

%\author[0000-0002-4355-6485]{Stefanie~M\"uhle}
%\affiliation{Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, D-53121 Bonn, Germany}(*)
%\email{muehle@astro.uni-bonn.de}

% Other authors.  These authors only appear on the full author list which
% appears on the last page of the article.  Order is alphabetical.

% \author[0000-0002-5828-7660]{Susanne Aalto}
% \affiliation{Department of Space, Earth, and Environment, Onsala Space Observatory, Chalmers University of Technology, Onsala Observatory, SE-439 92 Onsala, Sweden}
% %\email{saalto@chalmers.se}

\author[0000-0002-1316-1343]{Rebeca Aladro}
\affiliation{Max-Planck-Institut f\"ur Radioastronomie, Auf dem H\"ugel 69, 53121 Bonn, Germany}
% %\email{aladro@mpifr-bonn.mpg.de}

 \author[0000-0001-8064-6394]{Laura Colzi}
\affiliation{Centro de Astrobiolog\'ia (CSIC-INTA), Ctra. de Ajalvir Km. 4, 28850, Torrej\'on de Ardoz, Madrid, Spain}
\affiliation{INAF-Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy 5}
% %\email{lcolzi.astro@gmail.com}

% \author[0000-0001-8509-1818]{Gary A.~Fuller}
% \affiliation{Jodrell Bank Centre for Astrophysics, Department of Physics \& Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester, M13 9PL, UK}
% %\email{g.fuller@manchester.ac.uk}

% \author[0000-0003-0444-6897]{Santiago Garc\'{\i}a-Burillo}
% \affiliation{Observatorio Astron\'omico  Nacional (OAN-IGN), Observatorio de Madrid, Alfonso XII, 3, 28014-Madrid, Spain}
% %\email{s.gburillo@oan.es}

% \author[0000-0001-6431-9633]{Adam G.~Ginsburg}
% \affiliation{Department of Astronomy, University of Florida, Bryant Space Science Center, Stadium Road, Gainesville, FL 32611, USA}
% %\email{adamginsburg@ufl.edu}

% \author[0000-0002-2554-1837]{Thomas R.~Greve}
% \affiliation{Dept. of Physics and Astronomy, University College London, Gower Street, London WC1E6BT, UK}
% \affiliation{Cosmic Dawn Center}
% %\email{t.greve@ucl.ac.uk}

\author[0000-0001-6527-6954]{Kimberly L. Emig}
\altaffiliation{Jansky Fellow of the National Radio Astronomy Observatory}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Road,
  Charlottesville, VA  22903-2475, USA}

 \author[0000-0002-7495-4005]{Christian Henkel}
 \affiliation{Max-Planck-Institut f\"ur Radioastronomie, Auf dem H\"ugel   69, 53121 Bonn, Germany}
 \affiliation{Astronomy Department, Faculty of Science, King Abdulaziz
   University, P.~O.~Box 80203, Jeddah 21589, Saudi Arabia}
% %\email{chenkel@mpifr-bonn.mpg.de}



\author[0000-0003-3537-4849]{P. K. Humire}
\affiliation{Max-Planck-Institut f\"ur Radioastronomie, Auf dem H\"ugel 69, 53121 Bonn, Germany}
% %\email{phumire@mpifr-bonn.mpg.de} 

% \author[0000-0001-9162-2371]{Leslie K.~Hunt}
% \affiliation{INAF-Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125 Firenze, Italy}
% %\email{hunt@arcetri.astro.it}

% \author[0000-0001-9452-0813]{Takuma Izumi} 
% \affiliation{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan} 
% %\email{takuma.izumi@nao.ac.jp} 

% \author[0000-0002-4052-2394]{Kotaro Kohno (河野孝太郎)}
% \affiliation{Institute of Astronomy, Graduate School of Science,
% The University of Tokyo, 2-21-1 Osawa, Mitaka, Tokyo 181-0015, Japan}
% \affiliation{Research Center for the Early Universe, Graduate
% School of Science, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku,
% Tokyo 113-0033, Japan}
% %\email{kkohno@ioa.s.u-tokyo.ac.jp}

\author[0000-0001-9436-9471]{David S.~Meier}
\affiliation{New Mexico Institute of Mining and Technology, 801 Leroy Place, Socorro, NM 87801, USA}
\affiliation{National Radio Astronomy Observatory, PO Box O, 1003 Lopezville Road, Socorro, NM 87801, USA}
% %\email{david.meier@nmt.edu}

% \author{Taku Nakajima}
% \affiliation{Institute for Space-Earth Environmental Research, Nagoya University, Furo-cho, Chikusa-ku, Nagoya, Aichi 464-8601, Japan}
% %\email{nakajima@isee.nagoya-u.ac.jp}

% \author[0000-0003-0563-067X]{Yuri Nishimura}
% \affiliation{Institute of Astronomy, The University of Tokyo, 
% 2-21-1, Osawa, Mitaka, Tokyo 181-0015, Japan}
% \affiliation{ALMA Project, National Astronomical Observatory of Japan, 
% 2-21-1, Osawa, Mitaka, Tokyo 181-8588, Japan}
%% %\email{yuri@ioa.s.u-tokyo.ac.jp}

 \author[0000-0002-2887-5859]{V\'ictor M.~Rivilla}
 \affiliation{Centro de Astrobiolog\'ia (CSIC-INTA), Ctra. de Ajalvir Km. 4, 28850, Torrej\'on de Ardoz, Madrid, Spain}
 \affiliation{INAF-Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, I-50125, Florence, Italy 5}
% %\email{vmrivilla@gmail.com}

% \author[0000-0003-1946-8482]{Mamiko T.~Sato}
% \affiliation{Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Observatory, SE-439 92 Onsala, Sweden}
% %\email{mamiko@chalmers.se}

% \author[0000-0001-6788-7230]{Shuro Takano}
% \affiliation{Department of Physics, General Studies,
% College of Engineering, Nihon University, Tamura-machi,
% Koriyama, Fukushima 963-8642, Japan}
% %\email{takano.shuro@nihon-u.ac.jp}

 \author[0000-0001-5434-5942]{Paul P.~van der Werf}
 \affiliation{Leiden Observatory, Leiden University,
     PO Box 9513, NL - 2300 RA Leiden, The Netherlands}
 %\email{pvdwerf@strw.leidenuniv.nl}
 
% \author[0000-0002-8809-2725]{Yongxiong Wang (王永雄)}
% %\author[0000-0002-8809-2725]{Yongxiong Wang}
% \affiliation{Jodrell Bank Centre for Astrophysics, Department of Physics
% \& Astronomy, School of Natural Sciences, The University of Manchester,
% Oxford Road, Manchester, M13 9PL, UK}
% %\email{yongxiong.wang@postgrad.manchester.ac.uk}

\collaboration{20}{(ALMA Comprehensive High-resolution Extragalactic Molecular Inventory (ALCHEMI) collaboration)} 


==> AuthorList_n_Affliations.tex <==
          \author{K.-Y. Huang
          \inst{\ref{inst.Leiden}}
          \and S. Viti
          \inst{\ref{inst.Leiden},\ref{inst.UCL}}
          \and J. Holdship
          \inst{\ref{inst.Leiden}}
          \and S. Mart\'in \inst{\ref{inst.ESOChile},\ref{inst.JAO}}
          \and J. Mangum \inst{\ref{inst.NRAOCV}}
          \and N. Harada \inst{\ref{inst.NAOJ},\ref{inst.ASIAA}, \ref{inst.SOKENDAI}}
          \and S. Muller \inst{\ref{inst.ONSALA}}
          \and K. Sakamoto \inst{\ref{inst.ASIAA}}
%----------DATA REDUCTION
          \and K. Tanaka \inst{\ref{inst.KeioUniversity}}
          \and Y. Yoshimura \inst{\ref{inst.UTokio}}
          \and K. Nakanishi \inst{\ref{inst.NAOJ},\ref{inst.SOKENDAI}}
          \and S. M\"uhle \inst{\ref{inst.UBonn}}
          \and R. Herrero-Illana \inst{\ref{inst.ESOChile},\ref{inst.ICECSIC}}
%----------DATA REDUCTION
          \and D. S. Meier \inst{\ref{inst.NMIMT},\ref{inst.NRAOSocorro}}
          \and E. Caux \inst{\ref{inst.IRAP}}
          \and R. Aladro \inst{\ref{inst.MPIfR}}
          \and R. Mauersberger \inst{\ref{inst.MPIfR}}
          \and L. Colzi \inst{\ref{inst.CAB-INTA},\ref{inst.Arcetri}}
          \and V. M. Rivilla \inst{\ref{inst.CAB-INTA},\ref{inst.Arcetri}}
          \and M. Gorski \inst{\ref{inst.ONSALA}}
          \and K. M. Menten \inst{\ref{inst.MPIfR}}
          \and S. Aalto \inst{\ref{inst.ONSALA}}
          \and P. P.~van der Werf \inst{\ref{inst.Leiden}}
          \and K. L. Emig \inst{\ref{inst.NRAOCV}} 
          \thanks{Jansky Fellow of the National Radio Astronomy Observatory}
          }
          
          
%If there are too many authors, use \authorrunning
%\authorrunning{First Author et al.}

%


\institute{
\label{inst.Leiden}Leiden Observatory, Leiden University, PO Box 9513, NL - 2300 RA Leiden, The Netherlands
\and\label{inst.UCL}Department of Physics and Astronomy, University College London, Gower Street, London WC1E6BT, UK
\and\label{inst.MPIfR}Max-Planck-Institut f\"ur Radioastronomie, Auf-dem-H\"ugel 69, 53121 Bonn, Germany, \label{email}phumire@mpifr-bonn.mpg.de %\email{phumire@mpifr-bonn.mpg.de} \label{email}phumire@mpifr-bonn.mpg.de   
\and\label{inst.Abdulaziz}Astron. Dept., Faculty of Science, King Abdulaziz University, P.O. Box 80203, Jeddah 21589, Saudi Arabia
\and\label{inst.Xinjiang}Xinjiang Astronomical Observatory, Chinese Academy of Sciences, 830011 Urumqi, China
\and\label{inst.ESOChile}European Southern Observatory, Alonso de C\'ordova, 3107, Vitacura, Santiago 763-0355, Chile  
\and\label{inst.JAO}Joint ALMA Observatory, Alonso de C\'ordova, 3107, Vitacura, Santiago 763-0355, Chile
\and\label{inst.NRAOCV}National Radio Astronomy Observatory, 520 Edgemont Road, Charlottesville, VA 22903-2475, USA
\and\label{inst.NAOJ}National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan
\and\label{inst.ASIAA}Institute of Astronomy and Astrophysics, Academia Sinica, 11F of AS/NTU Astronomy-Mathematics Building, No.1, Sec. 4, Roosevelt Rd, Taipei 10617, Taiwan
\and\label{inst.SOKENDAI}Department of Astronomy, School of Science, The Graduate University for Advanced Studies (SOKENDAI), 2-21-1 Osawa, Mitaka, Tokyo, 181-1855 Japan
\and\label{inst.ONSALA}Department of Space, Earth and Environment, Chalmers University of Technology, Onsala Space Observatory, SE-43992 Onsala, Sweden
\and\label{inst.KeioUniversity}Department of Physics, Faculty of Science and Technology, Keio University, 3-14-1 Hiyoshi, Yokohama, Kanagawa 223--8522 Japan
\and\label{inst.UTokio}Institute of Astronomy, Graduate School of Science, The University of Tokyo, 2-21-1 Osawa, Mitaka, Tokyo 181-0015, Japan
\and\label{inst.UBonn}Argelander-Institut f\"ur Astronomie, Universit\"at Bonn, Auf dem H\"ugel 71, D-53121 Bonn, Germany
\and\label{inst.ICECSIC}Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Magrans, E-08193 Barcelona, Spain
\and\label{inst.IRAP}IRAP, Universit\'e de Toulouse, CNRS, UPS, CNES, Toulouse, France
\and\label{inst.CAB-INTA}Centro de Astrobiología (CSIC-INTA), Ctra. de Torrej\'on a Ajalvir km 4, 28850, Torrej\'on de Ardoz, Madrid, Spain       
\and\label{inst.Arcetri}INAF Osservatorio Astrofisico di Arcetri, Largo Enrico Fermi 5, I-50125 Firenze, Italy
\and\label{inst.NMIMT}New Mexico Institute of Mining and Technology, 801 Leroy Place, Socorro, NM 87801, USA
\and\label{inst.NRAOSocorro}National Radio Astronomy Observatory, PO Box O, 1003 Lopezville Road, Socorro, NM 87801, USA
}
